DialogVCS: Robust Natural Language Understanding in Dialogue System Upgrade

In the constant updates of the product dialogue systems, we need to retrain the natural language understanding (NLU) model as new data from the real users would be merged into the existent data accumulated in the last updates. Within the newly added data, new intents would emerge and might have semantic entanglement with the existing intents, e.g. new intents that are semantically too specific or generic are actually subset or superset of some existing intents in the semantic space, thus impairing the robustness of the NLU model. As the first attempt to solve this problem, we setup a new benchmark consisting of 4 Dialogue Version Control dataSets (DialogVCS). We formulate the intent detection with imperfect data in the system update as a multi-label classification task with positive but unlabeled intents, which asks the models to recognize all the proper intents, including the ones with semantic entanglement, in the inference. We also propose comprehensive baseline models and conduct in-depth analyses for the benchmark, showing that the semantically entangled intents can be effectively recognized with an automatic workflow.

==> table_bk.tex <==
\begin{table*}[h]
\centering
\small
\setlength\tabcolsep{3pt}
    \centering
        \begin{tabular}{cccccc}
    \toprule
    Model & ATIS-VCS & SNIPS-VCS & CrossWOZ-VCS & MultiWOZ-VCS\\
    \midrule
    Negative Sample & 87.14/87.40/86.87 & 93.73/94.30/93.16 & 65.54/97.97/49.24 & 86.62/86.19/87.06 \\
    Focal Loss & 86.43/84.17/88.81 & 95.90/95.85/95.95 & 92.48/97.00/88.37 & 86.86/85.26/88.53 \\
    Multi-Label &  &  &  &  \\
    % \midrule
    Upper Bound & & & & \\
    \bottomrule
    \end{tabular}
    \caption{ Main Results of Negative sample, Two-Step Negative sample, Focal Loss, Multi-Label, and Contrastive Learning Method in the four datasets: ATIS, SNIPS, CrossWOZ and MultiWOZ. All methods in ATIS, SNIPS and MultiWOZ datasets use the same backbone of BERT-base-uncased. All methods in CrossWOZ dataset use the same backbone of BERT-base-chinese. Metrics in this table are F1-Score, Precision and Recall.}
    \label{tab:main-results-arithmetic}
\vspace{-0.1in}
\end{table*}

\begin{table*}[h]
\centering
\small
\setlength\tabcolsep{3pt}
    \centering
        \begin{tabular}{cccccc}
    \toprule
    Model & ATIS & SNIPS & CrossWOZ & MultiWOZ\\
    \midrule
    Negative Sample & 87.14/76.37/23.63 & 93.73/94.30/93.16 & 65.54/42.97/57.03 & 86.62/82.79/17.21 \\
    Two-Step NS & 84.70/73.29/26.71 & 88.59/63.71/36.29 &  &  \\
    % \midrule
    Focal Loss & 86.43/77.05/22.95 & 95.90/92.86/7.14 & 92.48/90.34/19.66 & 87.52/85.85/14.15 \\
    % \midrule
    Multi-Label &  &  &  &  \\
    % \midrule
    Upper Bound & & & & \\
    \bottomrule
    \end{tabular}
    \caption{ Main Results of Negative sample, Two-Step Negative sample, Focal Loss, Multi-Label and Contrastive Learning Method in the four datasets: ATIS, SNIPS, CrossWOZ and MultiWOZ. All methods in ATIS, SNIPS and MultiWOZ datasets use the same backbone of BERT-base-uncased. All methods in CrossWOZ dataset use the same backbone of BERT-base-chinese. Metrics in this table are F1-Score, Exact Match Ratio and Zero One Loss.}
    \label{tab:main-results-arithmetic}
\vspace{-0.1in}
\end{table*}
